Linear Contextual Metaprogramming and Session Types

We explore the integration of metaprogramming in a call-by-value linear lambda-calculus and sketch its extension to a session type system. We build on a model of contextual modal type theory with multi-level contexts, where contextual values, closing arbitrary terms over a series of variables, may then be boxed and transmitted in messages. Once received, one such value may then be unboxed (with a let-box construct) and locally applied before being run. We present a series of examples where servers prepare and ship code on demand via session typed messages.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{D. Costa, R. Hu (Eds.): Programming Language Approaches to\\ Concurrency and Communication-cEntric Software 2024 (PLACES'24)\\
EPTCS 401, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.401.1}{10.4204/EPTCS.401.1}}


==> sections/figure-substitution-typing-judgment.tex <==
\begin{figure*}[t]
%\framebox[1.2\width]{$\substitutionTyping{\sigma}{\Delta}{\Gamma}$}
\begin{mathpar}
\inferrule* []
{ }
{\substitutionTyping{\emptySubstitution}{\emptySubstitution}{\Gamma}}

\inferrule* []
{\substitutionTyping{\sigma}{\Delta}{\Gamma_1} \\ \stageTransition{k}{\Gamma_1}{\Gamma_2}}
{\substitutionTyping{(\sigma, \lock_k)}{(\Delta, \lock)}{\Gamma_2}}

\inferrule* []
{\substitutionTyping{\sigma}{\Delta}{\Gamma} \\ \isterm{\Gamma}{M}{T}}
{\substitutionTyping{(\sigma, \singleSubstitution{x}{M})}{(\Delta, \binding{x}{T})}{\Gamma}}

\inferrule* []
{\substitutionTyping{\sigma}{\Delta}{\Gamma_1} \\ \Delta \neq \Delta', \lock \\ \stageTransition{k}{\Gamma_1}{\Gamma_2}}
{\substitutionTyping{(\sigma, \lock_k)}{\Delta}{\Gamma_2}}

\inferrule* []
{\substitutionTyping{\sigma}{\Delta}{\Gamma} \\ x \not\in \dom{\tail{\Delta}}}
{\substitutionTyping{(\sigma, \singleSubstitution{x}{M})}{\Delta}{\Gamma}}
\end{mathpar}
\caption{Substitution Typing Judgment}
\label{figure:substitution-typing-judgment}
\end{figure*}


==> sections/figure-substitutions-terms-abridged.tex <==
\begin{figure*}[t]
%% \framebox[1.2\width]{$M [\sigma]$}
%% \framebox[1.2\width]{$\overline{M} [\sigma]$}
\begin{alignat*}{4}
%c [\sigma] & = &&\ c\\
x [\sigma] & = && \begin{cases}M & \text{if } \singleSubstitution{x}{M} \in \tail{\sigma} \\ x & \text{otherwise}\end{cases}\\
(\abstraction{x}{T}{M}) [\sigma] & = &&\ \abstraction{x}{T}{(M [\sigma])} \text{ where } \singleSubstitution{x}{M'} \not\in \dom{\tail{\sigma}} \text{ and } x \not\in \fv{0}{\sigma}\\
(\application{M}{N}) [\sigma] & = &&\ \application{(M [\sigma])}{(N [\sigma])}\\
%\pair{M}{N} [\sigma] & = &&\ \pair{M [\sigma]}{N [\sigma]}\\
%(\pairDestructor{x}{y}{M}{N}) [\sigma] & = &&\ \pairDestructor{x}{y}{M [\sigma]}{N [\sigma]}\\
%(\new{S}) [\sigma] & = &&\ \new{S}\\
(\match{M}{l : N_l}{l \in L}) [\sigma] & = &&\ (\match{M [\sigma]}{l : N_l [\sigma]}{l \in L})\\
(\quo{\hat{\Gamma}}{M}) [\sigma] & = &&\ \quo{\hat{\Gamma}}{M [\sigma, \lock_1, id_{\hat{\Gamma}}]}\\
(\unq{k}{M}{\overline{N}}) [\sigma] & = &&\ \unq{\countFun{k}{\sigma}}{(M [\upFun{\sigma}{k}])}{\overline{N} [\sigma]}
%\overline{N} [\sigma] & = &&\ N_1 [\sigma], \ldots, N_n [\sigma] \text{ where } \overline{N} = N_1, \ldots, N_n
\end{alignat*}
\caption{Substitutions on Terms}
\label{figure:substitutions-terms}
\end{figure*}
%
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sections/figure-substitutions-terms.tex <==
\begin{figure*}[h!]
%% \framebox[1.2\width]{$M [\sigma]$}
%% \framebox[1.2\width]{$\overline{M} [\sigma]$}
\begin{alignat*}{4}
c [\sigma] & = &&\ c\\
x [\sigma] & = && \begin{cases}M & \text{if } \singleSubstitution{x}{M} \in \tail{\sigma} \\ x & \text{otherwise}\end{cases}\\
(\abstraction{x}{T}{M}) [\sigma] & = &&\ \abstraction{x}{T}{(M [\sigma])} \text{ where } \singleSubstitution{x}{M'} \not\in \dom{\tail{\sigma}} \text{ and } x \not\in \fv{0}{\sigma}\\
(\application{M}{N}) [\sigma] & = &&\ \application{(M [\sigma])}{(N [\sigma])}\\
\pair{M}{N} [\sigma] & = &&\ \pair{M [\sigma]}{N [\sigma]}\\
(\pairDestructor{x}{y}{M}{N}) [\sigma] & = &&\ \pairDestructor{x}{y}{M [\sigma]}{N [\sigma]}\\
(\new{S}) [\sigma] & = &&\ \new{S}\\
(\match{M}{l : N_l}{l \in L}) [\sigma] & = &&\ (\match{M [\sigma]}{l : N_l [\sigma]}{l \in L})\\
(\quo{\hat{\Gamma}}{M}) [\sigma] & = &&\ \quo{\hat{\Gamma}}{M [\sigma, \lock_1, id_{\hat{\Gamma}}]}\\
(\unq{k}{M}{\overline{N}}) [\sigma] & = &&\ \unq{\countFun{k}{\sigma}}{(M [\upFun{\sigma}{k}])}{\overline{N} [\sigma]}\\
\overline{N} [\sigma] & = &&\ N_1 [\sigma], \ldots, N_n [\sigma] \text{ where } \overline{N} = N_1, \ldots, N_n
\end{alignat*}
\caption{Substitutions on Terms}
%\label{figure:substitutions-terms}
\end{figure*}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

